Technical Debt and Waste in Non-Functional Requirements Documentation: An Exploratory Study

Background: To adequately attend to non-functional requirements (NFRs), they must be documented; otherwise, developers would not know about their existence. However, the documentation of NFRs may be subject to Technical Debt and Waste, as any other software artefact. Aims: The goal is to explore indicators of potential Technical Debt and Waste in NFRs documentation. Method: Based on a subset of data acquired from the most recent NaPiRE (Naming the Pain in Requirements Engineering) survey, we calculate, for a standard set of NFR types, how often respondents state they document a specific type of NFR when they also state that it is important. This allows us to quantify the occurrence of potential Technical Debt and Waste. Results: Based on 398 survey responses, four NFR types (Maintainability, Reliability, Usability, and Performance) are labelled as important but they are not documented by more than 22% of the respondents. We interpret that these NFR types have a higher risk of Technical Debt than other NFR types. Regarding Waste, 15% of the respondents state they document NFRs related to Security and they do not consider it important. Conclusions: There is a clear indication that there is a risk of Technical Debt for a fixed set of NFRs since there is a lack of documentation of important NFRs. The potential risk of incurring Waste is also present but to a lesser extent.

==> table_averages.tex <==

\begin{tabular}{llrrrr}
\toprule
             &      &           Mean (TD) &   Std (TD) &   Mean (W) &   Std (W) \\
\midrule
Process type & Agile &          26.59 &  0.09 &   7.54 &  0.03 \\
             & Hybrid &          20.28 &  0.06 &   9.81 &  0.03 \\
             & Plan-driven &          22.30 &  0.10 &   8.78 &  0.05 \\
             & Rather agile &          23.16 &  0.10 &  10.26 &  0.05 \\
             & Rather plan-driven &          18.57 &  0.06 &  12.32 &  0.04 \\\midrule
Project size & L &          20.93 &  0.06 &   9.96 &  0.03 \\
             & M &          20.50 &  0.07 &  11.49 &  0.04 \\
             & S &          24.01 &  0.08 &   8.27 &  0.02 \\\midrule
System class & BIS &          22.40 &  0.09 &   9.65 &  0.04 \\
             & HYB &          23.14 &  0.05 &   8.91 &  0.03 \\
             & SIES &          19.34 &  0.05 &  11.45 &  0.02 \\
\bottomrule
\end{tabular}


==> table_full.tex <==
\begin{tabular}{lllllllllll}
\toprule
             &   & variable & Compatibility & Maintainability &   Performance &   Portability &   Reliability &        Safety &      Security &     Usability \\
{} & system\_class & value &               &                 &               &               &               &               &               &               \\
\midrule
system\_class & BIS & I\_D+NI\_ND &  147 (72.77\%) &    112 (55.45\%) &  134 (66.34\%) &  165 (81.68\%) &  126 (62.38\%) &  152 (75.25\%) &  128 (63.37\%) &  134 (66.34\%) \\
             &   & I\_ND &   35 (17.33\%) &     75 (37.13\%) &   42 (20.79\%) &    18 (8.91\%) &   64 (31.68\%) &   39 (19.31\%) &   37 (18.32\%) &   52 (25.74\%) \\
             &   & NI\_D &     20 (9.9\%) &      15 (7.43\%) &   26 (12.87\%) &    19 (9.41\%) &    12 (5.94\%) &    11 (5.45\%) &   37 (18.32\%) &    16 (7.92\%) \\
             & HYB & I\_D+NI\_ND &   72 (71.29\%) &     68 (67.33\%) &   64 (63.37\%) &   77 (76.24\%) &   62 (61.39\%) &   73 (72.28\%) &   65 (64.36\%) &   68 (67.33\%) \\
             &   & I\_ND &   18 (17.82\%) &     29 (28.71\%) &   27 (26.73\%) &   17 (16.83\%) &   31 (30.69\%) &   17 (16.83\%) &   23 (22.77\%) &   25 (24.75\%) \\
             &   & NI\_D &   11 (10.89\%) &       4 (3.96\%) &     10 (9.9\%) &     7 (6.93\%) &     8 (7.92\%) &   11 (10.89\%) &   13 (12.87\%) &     8 (7.92\%) \\
             & SIES & I\_D+NI\_ND &   63 (66.32\%) &     68 (71.58\%) &   63 (66.32\%) &   71 (74.74\%) &    57 (60.0\%) &   74 (77.89\%) &   66 (69.47\%) &   64 (67.37\%) \\
             &   & I\_ND &   17 (17.89\%) &      19 (20.0\%) &   21 (22.11\%) &   11 (11.58\%) &   27 (28.42\%) &   12 (12.63\%) &   20 (21.05\%) &   20 (21.05\%) \\
             &   & NI\_D &   15 (15.79\%) &       8 (8.42\%) &   11 (11.58\%) &   13 (13.68\%) &   11 (11.58\%) &     9 (9.47\%) &     9 (9.47\%) &   11 (11.58\%) \\
process & Agile & I\_D+NI\_ND &   41 (65.08\%) &     34 (53.97\%) &   38 (60.32\%) &   45 (71.43\%) &   38 (60.32\%) &   46 (73.02\%) &    47 (74.6\%) &   43 (68.25\%) \\
             &   & I\_ND &    16 (25.4\%) &     25 (39.68\%) &   20 (31.75\%) &   10 (15.87\%) &   22 (34.92\%) &   14 (22.22\%) &   10 (15.87\%) &   17 (26.98\%) \\
             &   & NI\_D &     6 (9.52\%) &       4 (6.35\%) &     5 (7.94\%) &     8 (12.7\%) &     3 (4.76\%) &     3 (4.76\%) &     6 (9.52\%) &     3 (4.76\%) \\
             & Hybrid & I\_D+NI\_ND &   94 (69.63\%) &      86 (63.7\%) &   85 (62.96\%) &  107 (79.26\%) &   93 (68.89\%) &   103 (76.3\%) &   93 (68.89\%) &   94 (69.63\%) \\
             &   & I\_ND &   23 (17.04\%) &     41 (30.37\%) &   34 (25.19\%) &   17 (12.59\%) &   33 (24.44\%) &   19 (14.07\%) &   24 (17.78\%) &   28 (20.74\%) \\
             &   & NI\_D &   18 (13.33\%) &       8 (5.93\%) &   16 (11.85\%) &    11 (8.15\%) &     9 (6.67\%) &    13 (9.63\%) &   18 (13.33\%) &    13 (9.63\%) \\
             & Plan-driven & I\_D+NI\_ND &   28 (75.68\%) &     20 (54.05\%) &   27 (72.97\%) &   30 (81.08\%) &   26 (70.27\%) &   30 (81.08\%) &   21 (56.76\%) &   22 (59.46\%) \\
             &   & I\_ND &    5 (13.51\%) &     15 (40.54\%) &    5 (13.51\%) &    5 (13.51\%) &    9 (24.32\%) &    6 (16.22\%) &   11 (29.73\%) &   10 (27.03\%) \\
             &   & NI\_D &    4 (10.81\%) &       2 (5.41\%) &    5 (13.51\%) &     2 (5.41\%) &     2 (5.41\%) &      1 (2.7\%) &    5 (13.51\%) &    5 (13.51\%) \\
             & Rather agile & I\_D+NI\_ND &   67 (70.53\%) &     66 (69.47\%) &   62 (65.26\%) &    76 (80.0\%) &   49 (51.58\%) &   69 (72.63\%) &   55 (57.89\%) &   62 (65.26\%) \\
             &   & I\_ND &   17 (17.89\%) &     26 (27.37\%) &    19 (20.0\%) &     5 (5.26\%) &    38 (40.0\%) &   21 (22.11\%) &   24 (25.26\%) &   26 (27.37\%) \\
             &   & NI\_D &   11 (11.58\%) &       3 (3.16\%) &   14 (14.74\%) &   14 (14.74\%) &     8 (8.42\%) &     5 (5.26\%) &   16 (16.84\%) &     7 (7.37\%) \\
             & Rather plan-driven & I\_D+NI\_ND &   52 (76.47\%) &     42 (61.76\%) &   49 (72.06\%) &   55 (80.88\%) &   39 (57.35\%) &    51 (75.0\%) &   43 (63.24\%) &   45 (66.18\%) \\
             &   & I\_ND &    9 (13.24\%) &     16 (23.53\%) &   12 (17.65\%) &    9 (13.24\%) &   20 (29.41\%) &    8 (11.76\%) &   11 (16.18\%) &   16 (23.53\%) \\
             &   & NI\_D &    7 (10.29\%) &     10 (14.71\%) &    7 (10.29\%) &     4 (5.88\%) &    9 (13.24\%) &    9 (13.24\%) &   14 (20.59\%) &    7 (10.29\%) \\
project\_size & L & I\_D+NI\_ND &   88 (71.54\%) &     79 (64.23\%) &   85 (69.11\%) &   96 (78.05\%) &   82 (66.67\%) &   90 (73.17\%) &   80 (65.04\%) &   80 (65.04\%) \\
             &   & I\_ND &   22 (17.89\%) &     35 (28.46\%) &   27 (21.95\%) &    15 (12.2\%) &   33 (26.83\%) &   19 (15.45\%) &    23 (18.7\%) &   32 (26.02\%) \\
             &   & NI\_D &   13 (10.57\%) &       9 (7.32\%) &    11 (8.94\%) &    12 (9.76\%) &      8 (6.5\%) &   14 (11.38\%) &   20 (16.26\%) &    11 (8.94\%) \\
             & M & I\_D+NI\_ND &   95 (69.85\%) &     86 (63.24\%) &   83 (61.03\%) &  109 (80.15\%) &   81 (59.56\%) &   99 (72.79\%) &   88 (64.71\%) &   99 (72.79\%) \\
             &   & I\_ND &   23 (16.91\%) &     39 (28.68\%) &   30 (22.06\%) &    13 (9.56\%) &   41 (30.15\%) &   27 (19.85\%) &   25 (18.38\%) &   25 (18.38\%) \\
             &   & NI\_D &   18 (13.24\%) &      11 (8.09\%) &   23 (16.91\%) &   14 (10.29\%) &   14 (10.29\%) &    10 (7.35\%) &   23 (16.91\%) &    12 (8.82\%) \\
             & S & I\_D+NI\_ND &   99 (71.22\%) &     83 (59.71\%) &   93 (66.91\%) &   108 (77.7\%) &   82 (58.99\%) &  110 (79.14\%) &   91 (65.47\%) &   87 (62.59\%) \\
             &   & I\_ND &   25 (17.99\%) &     49 (35.25\%) &   33 (23.74\%) &   18 (12.95\%) &   48 (34.53\%) &   22 (15.83\%) &   32 (23.02\%) &   40 (28.78\%) \\
             &   & NI\_D &   15 (10.79\%) &       7 (5.04\%) &    13 (9.35\%) &    13 (9.35\%) &     9 (6.47\%) &     7 (5.04\%) &   16 (11.51\%) &    12 (8.63\%) \\
\bottomrule
\end{tabular}
